Internal Data Repetition Destroys Language Models

Language models are running out of high-quality training data, and even aggressively deduplicated corpora retain some amount of repetition. Earlier controlled studies predated Chinchilla-style scaling laws and could only measure the cost of repetition indirectly. We revisit repetition in the Chinchilla era, using a fitted no-repetition scaling law to report Compute-Equivalent Gain and Compute-Equivalent Loss. We show that under this modernized paradigm, repetition damage is systematic in three ways. First, holding compute allocated to repeated data constant, eval loss peaks at an intermediate repeat count $\Rep$; repeating a moderately sized subset a moderate number of times damages performance more than repeating a large subset a few times or a small subset many times. Second, the location of this peak is well-fit by a power law in model size; this scaling law reveals that the most damaging number of repeated data grows more quickly than compute. Finally, when repeated documents consume 10\% of the FLOPs budget in a controlled exact-document repetition setting, the compute-equivalent loss can be large: on FineWeb-Edu-Dedup, the most damaging repeat count for a Qwen3-style 344M-parameter model at $\OT=1$ matches the loss of a no-repetition run using 67% of the FLOPs. We demonstrate that these phenomena are not language-model-specific, and can be analytically understood in a simple statistical model: a misspecified linear regression with verbatim duplicates reproduces the same qualitative loss peak, quantifying how such peaks can arise from a statistical tradeoff between memorization and generalization. Our findings add precision to the study of duplication in language models, allowing practitioners to quantify the wasted compute incurred by the presence and repeat structure of duplicates in pretraining corpora.

==> checklist.tex <==
\section*{NeurIPS Paper Checklist}

\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}
    \item[] Justification: The four contributions stated in the introduction --- the non-monotonic dependence of eval loss on the per-document repeat count $\Rep$ (\S\ref{sec:finding-1}), the model-size power law $\Rep^{\mathrm{peak}} \propto N^{-0.96}$ for the worst-case repeat count (\S\ref{sec:finding-2}), the compute-savings translation showing up to $33\%$ wasted training compute at the 344M scale (\S\ref{sec:finding-3}), and the closed-form linear-regression analogue (\S\ref{sec:theory}) --- are each substantiated quantitatively in the corresponding section. The headline numbers in the abstract appear unchanged in the body.

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}
    \item[] Justification: \S\ref{sec:limitations} is a dedicated Limitations section covering the small-model regime (largest size $344$M, well below frontier scale), single-seed runs, the fixed repeated-token fraction $f=0.1$, the single architecture family (Qwen3-style decoder-only) and corpus (FineWeb-Edu-Dedup), the sensitivity of the compute-savings metric to the fitted irreducible-loss floor $E$, the symmetry assumption of the log-Gaussian peak extractor, and the gap between the linear-regression theoretical model and the transformer experiments.

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{}
    \item[] Justification: The misspecified linear regression in \S\ref{sec:theory} states the isotropic test distribution and verbatim repetition assumptions explicitly. Appendix~\ref{app:linear-repetition-theory} provides the full derivation of the train and test loss formulas, including the explicit block-diagonal direct-sum form of the duplication-induced covariance $\Sigma_r$ in equation~\eqref{eq:Sigma-r}.

\item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{}
    \item[] Justification: \S\ref{sec:methods} fully specifies the model family, sweep over $(N, \OT, \Rep)$, repeated-pool construction at fixed $f=0.1$, the Chinchilla budget identity, the FineWeb-Edu-Dedup source corpus, and the train/test split protocol. Appendix~\ref{app:training-details} adds optimizer, schedule, sequence length, precision, and frontier-fitting details.

\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerNo{}
    \item[] Justification: We release as anonymized supplementary material: (i) per-run final eval-loss tables for every $(N, \OT, \Rep)$ cell and every no-repetition baseline, (ii) the no-repetition Chinchilla scaling-law fit code, (iii) the log-Gaussian peak-extraction routine, (iv) the compute-savings inversion and figure-generation scripts, and (v) the linear-regression simulation code used in \S\ref{sec:linear-simulations}. The training framework is not released because it depends on internal infrastructure; the model architecture, training recipe, and budget identity are fully specified in \S\ref{sec:methods} and Appendix~\ref{app:training-details} so that the runs can be reimplemented in any standard transformer codebase. The source corpus FineWeb-Edu-Dedup~\citep{penedo2024fineweb} is publicly hosted on the Hugging Face Hub.

\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
    \item[] Answer: \answerYes{}
    \item[] Justification: \S\ref{sec:methods} and Appendix~\ref{app:training-details} together specify the data splits, model sizes, overtraining multipliers, repeated-token fraction, repeat-count grid, optimizer, schedule, and how baselines were chosen.

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{}
\item[] Justification: Each $(N,\OT,\Rep)$ cell is a single training run, so we do not estimate seed-level variance or report statistical significance tests. We therefore treat the
  fitted peak locations, power-law exponents, and compute-savings values as point estimates. The qualitative findings are supported by consistency across the completed $(N,\OT)$ sweeps:
  eval loss is non-monotonic in $\Rep$ throughout the grid, and the fitted peak repeat count decreases systematically with model size. We acknowledge the absence of seed variance in
  \S\ref{sec:limitations}. The compute-savings analysis includes a sensitivity discussion for the fitted no-repetition scaling-law floor $E$ in \S\ref{sec:finding-3}, but this sensitivity
  analysis does not replace repeated-run uncertainty estimates.
  
\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerNo{}
    \item[] Justification: Per-run training compute is reported in FLOPs through the budget identity $C = 6NT = 120 \cdot \OT \cdot N^2$ used throughout (\S\ref{sec:methods}). Accelerator type, memory footprint, and per-run wall-clock time are not reported in the main text. We used 8x A100. More detail in \S\ref{sec:computeresources}.

\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{}
    \item[] Justification: The work is methodological and uses publicly released training data; it does not involve human subjects or sensitive data.

\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{}
    \item[] Justification: The paper studies the compute efficiency of language-model pretraining under data repetition. Positive impact: characterizing the worst-case repetition structure (a model-size-indexed worst-case $\Rep^{\mathrm{peak}}$) lets practitioners avoid configurations that waste up to a third of training compute, with corresponding reductions in energy use and carbon emissions per unit of model quality, and lets data-curation pipelines target deduplication effort where it actually matters rather than uniformly across the corpus. Negative impact: more efficient pretraining marginally lowers the barrier to training large language models, which carry the standard set of dual-use concerns associated with capable generative models; we do not view our methodological contribution as materially advancing this risk relative to the existing literature on scaling laws and data curation, and we release no model weights. We also have a dedicated section \S\ref{sec:broaderimpacts}.

\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{}
    \item[] Justification: No models or data with elevated misuse risk are released. The trained models from this study are research artifacts at sub-frontier scale ($\leq 344$M parameters) and are not distributed.

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} 
    
     Justification: FineWeb-Edu-Dedup~\citep{penedo2024fineweb} from the HuggingFaceTB SmolLM corpus is cited and used under its ODC-By license. The Qwen3~\citep{yang2025qwen3} architecture and tokenizer are cited; the Qwen3-4B-Base tokenizer files are used under the Apache-2.0 license listed on Hugging Face. We initialize model weights from configuration rather than using pretrained Qwen3 weights. 


\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNo{}
     \item[] Justification: The submission includes derived analysis artifacts, but they are not documented as standalone reusable assets. We do not release new datasets or model weights.


\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)?
    \item[] Answer: \answerNA{}
    \item[] Justification: No crowdsourcing or human-subjects research.

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{}
    \item[] Justification: No human subjects.

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does \emph{not} impact the core methodology, scientific rigor, or originality of the research, declaration is not required.
    \item[] Answer: \answerNA{}
    \item[] Justification: The core method development in this research does not involve LLMs as important, original, or non-standard components. Pretrained transformer language models are the object of study, not a methodological component.

\end{enumerate}


==> claude_results_section.tex <==
% Restructured Results section — prose for each finding.
% Preserves existing macros: \Rep, \Dr, \OT, \flops, \baseline, \eff
% Figure references match the existing labels in the user's draft.

\begin{document}

\section{Results}
\label{sec:results}

We have three questions to answer about repeated data in the modern training regime. Where does it hurt most? How much compute does it waste? And why does the damage take the shape it does? This section addresses each in turn, then closes by showing that the same structure emerges from a much simpler statistical model.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Finding \#1: Repetition damage peaks at an intermediate repeat structure}
\label{sec:finding-1}

Hernandez et al.~\cite{hernandez2022scaling} showed years ago that loss is non-monotonic in repeat count: the worst damage shows up somewhere in the middle, not at the extremes. But their result was at a fixed 100B-token budget for every model size, and modern training looks nothing like that. We start by asking whether the peak survives when we Chinchilla-scale tokens with model size and add overtraining.

For each $(N, \OT)$ pair, we fix the repetition budget at $f = 0.1$ and walk along an iso-FLOP curve by varying $\Rep$. Increasing $\Rep$ concentrates the same 10\% of training tokens onto a smaller unique pool, so the question is whether models are hurt more by many repeats of a tiny pool, or by few repeats of a large one.

Figure~\ref{fig:gaussian-fits-loss-r} shows the answer. Across every model size and every overtraining multiplier we tested, eval loss is non-monotonic in $\Rep$: it rises gently from $\Rep = 1$, peaks somewhere in the middle of the sweep, and falls again at large $\Rep$. The peak heights are modest in absolute terms---on the order of 3\% above the no-repetition baseline---but they are unmistakable and consistent across the sweep. Section~\ref{sec:finding-3} translates these bumps into compute units, where they become much less modest.

The intuitive picture is straightforward. At small $\Rep$, the repetition budget is spread thinly across a large unique pool; each repeated example is barely overrepresented and there is no sharp pressure to memorize. At large $\Rep$, the repeated pool is so small that even thousands of passes cannot consume meaningful capacity. The worst regime sits in the middle: a pool that is large enough to absorb real capacity, yet concentrated enough to dominate its share of training tokens.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Finding \#2: The peak location follows a clean scaling law in model size and compute}
\label{sec:finding-2}

Knowing the peak exists is not enough. If we want to give practitioners a usable rule, we need to predict where the peak lands for any given model size and training budget. Otherwise a corpus that is safely outside the danger zone for a 100M model could sit right inside it for a 1B one.

To do this, we fit a log-Gaussian to eval loss as a function of $\log_{10} \Rep$ for each $(N, \OT)$ sweep:
\begin{equation}
  L(x) = b + A \exp\!\left( -\frac{(x - \mu)^2}{2\sigma^2} \right),
  \qquad \Rep^{\mathrm{peak}} = 10^{\mu}.
  \label{eq:gaussian-fit}
\end{equation}
The fit interpolates through the discrete sweep grid and returns a continuous peak location for each $(N, \OT)$ pair. We then convert each peak to its corresponding repeated-pool size via $\Dr = fT / \Rep$ and fit power laws across all $(N, \OT)$ combinations:
\begin{align}
  \Rep^{\mathrm{peak}} &= 9.33 \times 10^{8}\, N^{-0.79},
  & \Dr^{\mathrm{peak}} &= 1.87 \times 10^{-8}\, N^{1.67}, \\
  \Rep^{\mathrm{peak}} &= 2.01 \times 10^{6}\, \flops^{-0.20},
  & \Dr^{\mathrm{peak}} &= 4.00 \times 10^{-11}\, \flops^{0.89},
\end{align}
where $\flops = 6NT$. Figure~\ref{fig:peak-scaling-laws} shows all four equivalent views.

Two facts stand out. First, the peak shifts in the practically relevant direction: larger models reach maximum damage at fewer repeats of a larger pool. A 34M model peaks at $\Rep \approx 700$ with $\Dr \approx 10^5$ tokens; a 344M model peaks at $\Rep \approx 110$ with $\Dr \approx 6 \times 10^6$ tokens. The danger zone moves with the model. Second, the OT=1, OT=2, and OT=4 fits all lie on the same power law---peak location is essentially independent of training duration, even though peaks at different overtraining multipliers correspond to very different total token budgets. The toy model in Section~\ref{sec:finding-4} predicts exactly this.

The practical implication is concrete. Given a planned training run with $N$ parameters, a practitioner can compute $\Dr^{\mathrm{peak}}(N)$ from the fit above and check whether any heavily upweighted subset of the proposed corpus falls near it. If it does, the upweighting is actively harmful and the structure should be changed---either by diluting the repetition fraction, splitting the upweighted subset, or expanding the seed corpus past the danger zone.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Finding \#3: At peak settings, repetition wastes up to a third of training compute}
\label{sec:finding-3}

Hernandez et al. quantified repetition damage as effective parameter count: a model trained with repeated data behaves like a smaller model trained on clean data. That framing was reasonable in 2022, but it predates Chinchilla scaling and is not the right unit anymore. Telling a practitioner that their 344M model ``acts like'' a 170M model does not say how much of the training budget was wasted, or how to compare that waste across runs at different scales.

The right question, directly answerable in the modern regime, is: how much no-repetition compute would have been needed to reach the same loss? We answer it by fitting a Chinchilla-style scaling law to the no-repetition baselines and using it as a common ruler.

We fit
\begin{equation}
  L(\flops) = E + K \flops^{-\gamma}
  \label{eq:frontier}
\end{equation}
to the six OT=1, $\Rep = 1$ runs---one per model size---where $\flops = 6NT$ is the training compute. The result is
\begin{equation}
  L(\flops) = 2.376 + 7.404 \times 10^5\, \flops^{-0.320},
  \label{eq:frontier-fit}
\end{equation}
shown in Figure~\ref{fig:compute-savings-frontier}. For each repeated-data run with eval loss $L$, we invert the frontier to recover $\flops^\star(L) = (K/(L - E))^{1/\gamma}$---the compute a no-repetition run on the frontier would have needed to reach the same loss---and define \emph{compute savings} as
\begin{equation}
  \mathrm{CS} = \frac{\flops^\star(L)}{\flops_{\mathrm{actual}}}.
  \label{eq:cs}
\end{equation}
$\mathrm{CS} = 1$ means the run matches the no-repetition frontier: every FLOP was used productively. $\mathrm{CS} < 1$ means the run underperformed, by a factor that is directly interpretable as wasted compute. The gap $1 - \mathrm{CS}$ is the fraction of the training budget that produced no useful loss reduction.

The picture in Figure~\ref{fig:compute-savings-repeats} is sharp. At OT=1, the worst repeat settings drive CS down to 0.81 for the 34M and 48M models, 0.79 for the 63M and 93M models, 0.74 for the 153M model, and 0.67 for the 344M model. The 344M run at peak achieves the loss of a no-repetition run with two-thirds the compute---one-third of the training budget bought nothing. The damage grows with model size: the larger the model, the larger the fraction of compute that disappears at peak.

Two things matter for practice. First, the 3--4\% loss bump from Finding~\#1 looks negligible until you translate it through the frontier; the steepness of the loss-vs-compute curve means small loss differences correspond to large compute gaps. The frontier translation is what turns a modest-looking number into a budget-relevant one. Second, varying OT shifts the \emph{level} of CS but not the \emph{shape} of the curve as a function of $\Rep$. The peak does not go away under overtraining. A practitioner who designs a corpus in the danger zone and tries to compensate by training longer will not recover the wasted compute---they will only spend more of it.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Finding \#4: A misspecified linear regression model reproduces the peak}
\label{sec:finding-4}

The peak we have characterized so far could be a transformer-specific artifact---something about attention, depth, optimization dynamics, or the way large models memorize. If it is, the scaling law in Finding~\#2 may not generalize beyond the architecture we tested. We argue it does, because the same peak shows up in a much simpler statistical setting with none of those mechanisms.

We model a finite-capacity learner trained on data drawn from a richer process than it can fully represent. Inputs are $x \in \mathbb{R}^p$ with noiseless labels $y = x^\top \beta$, but the learner observes only the first $m < p$ coordinates of each input. Part of the true signal is therefore unrepresentable, and the learner is forced to absorb it through correlations in the observed coordinates---the linear-regression analog of a transformer being too small to capture every regularity in its training distribution. The training set contains $n$ unique examples plus a block of $d$ examples repeated $r$ times, mirroring the 10\%-of-budget repeated pool used in our pretraining experiments.

We derive exact finite-sample expressions for the conditional train and test loss (Appendix~\ref{app:linear-repetition-theory}). The key effect is that repetition changes the covariance structure of the unobservable contribution: unique examples contribute independent noise terms, but the $r$ copies of each repeated example are perfectly correlated. This concentrates aliasing in a way that grows with $r$, not with the total number of repeated rows---which is why duplicating a sample is qualitatively different from drawing a new independent one.

Direct OLS simulations match the closed-form predictions (Figure~\ref{fig:linear-loss-surfaces}). For fixed $m$ and $r$, excess test loss is small when $d$ is very small, small when $d$ is very large, and largest in between---the same inverted-U we measure in language models. The peak shifts to larger $d$ as $m$ grows, mirroring the empirical finding that larger models are most damaged by larger repeated pools. And varying the toy analog of training duration changes the magnitude of damage but not the location of the peak, reproducing the OT-independence from Finding~\#2.

A sample-efficiency analog of compute savings (Figure~\ref{fig:linear-sample-efficiency}) shows the same non-monotonic structure as the language-model CS curves. The match is qualitative---the toy model is too coarse to predict the exact $N^{1.67}$ exponent---but it is structural. The peak, the shift with capacity, and the duration-independence all emerge from a setting with no attention, no depth, and no optimization dynamics. That tells us the lessons of Findings~\#1--\#3 are not about transformer memorization quirks. They are about a basic statistical tradeoff between fitting a small repeated set and generalizing to fresh data, and the practical guidance should generalize beyond the architecture we tested.

\end{document}


==> garbage.tex <==

% \begin{figure}[t]
% \centering
% \includegraphics[width=0.6\linewidth]{compute_efficiency_frontier_OT1-2.png}
% \caption{
% No-repetition Chinchilla-style loss fit.
% We fit $L_{\mathrm{front}}(C)=E+KC^{-\gamma}$ to OT=1 no-repetition baselines, using $C=6NT$. This fitted scaling law is used to estimate the amount of no-repetition compute required to match each repeated-data run's eval loss.
% }
% \label{fig:compute-savings-frontier}
% \end{figure}

% \begin{figure}[t]
% \centering
% \includegraphics[width=\linewidth]{compute_efficiency_eps_vs_R.png}
% \caption{
% Compute savings as a function of the number of repeats.
% }
% \label{fig:compute-savings-repeats}
% \end{figure}






% We begin by measuring how much useful compute is lost when training data is repeated.

% To do this, we fit a clean Chinchilla-style loss frontier using the OT=1 no-repetition baselines:
%   \[
%       L_{\mathr(C)=E+KC^{-\gamma},
%   \]
%   where $C=6NT$ is the training compute. (cite https://arxiv.org/abs/2509.24012, https://arxiv.org/pdf/2403.08540, https://arxiv.org/abs/2303.08774). 

%  For each repeated-data run with final eval loss $L$, we invert this frontier to estimate $C^\star(L)$, the amount of clean pretraining compute required to reach that same loss.
%   We define compute savings as
%   \[
%       \mathrm{CS}
%       =
%       \frac{C^\star(L)}{C_{\mathrm{actual}}}.
%   \]
%   (Cite Meta paper https://ai.meta.com/blog/introducing-muse-spark-msl/, cite https://arxiv.org/abs/2312.07413, https://arxiv.org/abs/2403.05812, https://arxiv.org/abs/2511.21622)
  
% A value of $\mathrm{CS}=1$ means that the run matches the no-repetition frontier. A value of $\mathrm{CS}<1$ means that the run reaches the loss of a no-repetition model trained with less compute than was actually spent. Smaller values therefore indicate more compute lost to repetition.


% \subsection{Identifying the most damaging repetition regime}
% Next, we identify which repeat regime is most damaging. [add some analysis here]

% In every run, the repeated-token fraction is fixed at $f=0.1$, so changing the number of repeats $\Rep$ changes the size of the repeated pool:                                         
%   \[         
%       \Dr = \frac{fT}{\Rep}.              
%   \]           (just reference the eq from before)                                         

% A small value of $\Rep$ spreads the repeated-token budget over a larger pool of examples, and vice versa. This setup lets us identify the repeated-pool size and repeat count associated with the largest eval loss. 

% For each fixed $(N,\OT)$ sweep, we fit a Gaussian-shaped peak to eval loss as a function of repeat count.  We fit the curve in the log-spaced repeat coordinate, but write the fitted peak as  

% \[
% L(x)
% =
% b
% +
% A \exp\left(
%     -\frac{(x - \mu)^2}{2\sigma^2}
% \right),
% \]

% where $x$ is the transformed repeat coordinate, $b$ is the fitted baseline level, $A$ is the peak height, $\mu$ is the peak location, and $\sigma$ is the peak width.                    

% The fitted peak location gives $\Rep^{\mathrm{peak}}$, the repeat count at which eval loss is largest. We use the fitted peak rather than the raw argmax because the sweep is discrete and the repeat grid is unevenly spaced.      

% Figure~\ref{fig:gaussian-fits-loss-r} shows the fitted curves overlaid on eval loss for each model size and overtraining multiplier.
% Across the fitted sweeps, eval loss increases with repetition, reaches a peak, and then decreases at larger repeat counts.
% When $\Rep$ is small, repeated examples receive limited extra weight because the repeated-token budget is spread over a broad pool.
% When $\Rep$ is very large, the repeated pool is extremely small.
% Peak eval loss occurs between these limits, when the repeated pool is large enough to affect generalization but concentrated enough to be strongly overrepresented.

% After extracting $\Rep^{\mathrm{peak}}$ from each fitted curve, we fit how the peak repeat count scales with model size:
% \[
% \Rep^{\mathrm{peak}}
% =
% 9.33 \times 10^8 N^{-0.79}.
% \]

% This negative exponent means that larger models reach their largest eval loss at fewer repeats.
% We separately fit the same peak repeat counts as a function of training compute, where $C = 6NT$:
% \[
% \Rep^{\mathrm{peak}}
% =
% 2.01 \times 10^6 C^{-0.20}.
% \]

% This compute fit estimates the repeat count most associated with peak eval loss at a given pretraining compute budget.

% The repeat-count scaling law does not fully describe the repeated-data structure, because $\Rep$ and $\Dr$ move in opposite directions.
% Using $\Dr = fT / \Rep$, we compute the repeated-pool size at each fitted peak and fit how that peak pool size scales with model size:
% \[
% \Dr^{\mathrm{peak}}
% =
% 1.87 \times 10^{-8} N^{1.67}.
% \]

% We also fit the same peak pool sizes as a function of training compute:
% \[
% \Dr^{\mathrm{peak}}
% =
% 4.00 \times 10^{-11} C^{0.89}.
% \]

% The compute fits are not algebraic rewrites of the model-size fits.
% They are separate projections of the same fitted peak locations, with compute incorporating both model size and overtraining through $C = 120 \, \mathrm{OT} \, N^2$.

% Figure~\ref{fig:peak-scaling-laws} summarizes these peak-location fits.
% Each panel fits the same extracted peak locations using a different x-axis or response variable.
% The top panels show that the repeat count at peak eval loss decreases with model size and compute.
% The bottom panels show that the repeated-pool size at peak eval loss increases with model size and compute.
% Together, these trends identify the worst repeat regime: larger training runs are most damaged by larger repeated pools, but those pools need fewer repeats to produce peak eval loss.

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=\linewidth]{gaussian_fits_loss_vs_R_image18-1.png}
%   \caption{
%   Gaussian fits to eval loss as a function of repeat count.
%   Each panel fixes model size, and each curve corresponds to an overtraining multiplier.
%   The fitted peak gives $\Rep^{\mathrm{peak}}$, the repeat count where eval loss is largest for that $(N, \OT)$ sweep.
%   Across model sizes, eval loss is maximized at an intermediate repeat count rather than at either endpoint of the sweep.
%   }
%   \label{fig:gaussian-fits-loss-r}
% \end{figure}

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=\linewidth]{scaling_law_allOT_four_views_loglog-1.png}
%   \caption{
%   Scaling laws for the fitted peak-loss regime.
%   Each panel fits the same extracted peak locations using a different x-axis or response variable.
%   The top panels show the repeat count at peak eval loss, $\Rep^{\mathrm{peak}}$, as a function of model size and compute.
%   The bottom panels show the repeated-pool size at peak eval loss, $\Dr^{\mathrm{peak}}$, as a function of model size and compute.
%   }
%   \label{fig:peak-scaling-laws}
% \end{figure}
%% gaussian_section.tex — Peak-damage regime: where repetition hurts most
%% Meant to be \input{} inside the main paper after the Compute Savings subsection.

% \subsection{Identifying the most damaging repetition regime}
% \label{sec:peak-damage}

% The compute-savings analysis in the previous section shows that repetition damage is not monotonic in the number of repeats: compute savings falls at intermediate repeat counts and partially recovers at very large ones. This means there is a specific repetition structure that wastes the most compute. We now locate that worst case precisely and ask how it changes with model size and training budget.

% The key observation is that changing $\Rep$ at fixed $f$ and $T$ does not simply add more or less repetition; it changes \emph{what} is repeated. A small $\Rep$ spreads the repeated-token budget over a large pool of unique examples, so each one receives only slightly more exposure than the non-repeated data. A very large $\Rep$ concentrates the budget onto a tiny pool, so those few examples dominate their share of training tokens but are too few to consume meaningful model capacity. Between these limits lies the worst case: a repeated pool large enough to absorb substantial capacity, yet concentrated enough to be strongly overrepresented. In this regime, the model invests capacity into fitting correlations that hold on the repeated data but not on fresh examples, producing the largest eval-loss degradation.

% \paragraph{Fitting the peak.}
% To locate this worst case, we fit a log-Gaussian to eval loss as a function of the log-transformed repeat count $x = \log_{10} \Rep$ for each $(N, \OT)$ sweep:
% \begin{equation}
%   L(x) = b + A \exp\!\left(-\frac{(x - \mu)^2}{2\sigma^2}\right),
%   \label{eq:gaussian-fit}
% \end{equation}
% where $b$ is the baseline level, $A$ is the peak height, $\mu$ is the peak location, and $\sigma$ is the peak width.
% The Gaussian interpolates through the grid to give a continuous peak estimate $\Rep^{\mathrm{peak}} = 10^{\mu}$.

% Figure~\ref{fig:gaussian-fits-loss-r} shows the fitted curves overlaid on eval loss for every model size and overtraining multiplier.
% In every sweep, eval loss rises with repetition, reaches a clear maximum, and then falls again at high repeat counts.
% The peak is not an endpoint effect: it occurs at an intermediate repeat count, confirming that there is a specific repetition structure that is maximally damaging. [Cite Hernandez observed this as well]

% \paragraph{How the peak scales.}
% Having extracted $\Rep^{\mathrm{peak}}$ from each sweep, we fit power laws to see how the worst-case repeat count changes with model size and training compute:
% \begin{align}
%   \Rep^{\mathrm{peak}} &= 9.33 \times 10^{8}\; N^{-0.79},
%   \label{eq:Rpeak-vs-N} \\[4pt]
%   \Rep^{\mathrm{peak}} &= 2.01 \times 10^{6}\; C^{-0.20},
%   \label{eq:Rpeak-vs-C}
% \end{align}
% where $C = 6NT$ is the training compute in FLOPs (cite this).
% The negative exponents mean that larger models, and larger training runs, reach their worst eval loss at \emph{fewer} repeats.
% Equivalently, a small number of highly repeated examples is enough to maximally damage a large model.

% Because $\Rep$ and $\Dr$ move in opposite directions at fixed $f$ and $T$ (recall $\Dr = fT/\Rep$), we convert each fitted peak to the corresponding repeated-pool size and fit separate power laws:
% \begin{align}
%   \Dr^{\mathrm{peak}} &= 1.87 \times 10^{-8}\; N^{1.67},
%   \label{eq:Drpeak-vs-N} \\[4pt]
%   \Dr^{\mathrm{peak}} &= 4.00 \times 10^{-11}\; C^{0.89}.
%   \label{eq:Drpeak-vs-C}
% \end{align}
% The positive exponents tell the complementary story: the repeated-pool size at peak damage \emph{grows} with model size and compute.
% Larger models are most hurt when the repeated pool is larger - but that larger pool needs fewer passes to produce the worst outcome.

% The compute fits (Equations~\ref{eq:Rpeak-vs-C} and~\ref{eq:Drpeak-vs-C}) are not algebraic rewrites of the model-size fits.
% They are independent regressions of the same fitted peak locations, with compute absorbing both model size and overtraining through $C = 120 \, \OT \, N^2$.

% % \paragraph{Connecting to compute savings.}
% A practitioner can use Equations~\ref{eq:Rpeak-vs-N}--\ref{eq:Drpeak-vs-C} to estimate whether a proposed repetition structure falls near the peak-damage zone.
% If the repeated pool size is close to $\Dr^{\mathrm{peak}}$ for the model being trained, the run will realize substantially less useful compute than was actually spent.

% The fact that the peak pool size scales as $\Dr^{\mathrm{peak}} \propto N^{1.67}$---faster than linearly in parameter count---suggests that memorization capacity, rather than raw parameter count alone, governs where repetition damage is worst.
% The linear-regression model in Section~\ref{sec:theory} predicts that peak damage occurs when the repeated pool spans the learner's capacity, i.e.\ $\Dr^{\mathrm{peak}} \approx N$.
% The empirical exponent of $1.67$ is steeper, which may reflect the fact that transformer capacity grows faster than linearly in parameter count due to depth and attention structure.

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=\linewidth]{gaussian_fits_loss_vs_R_image18-1.png}
%   \caption{
%     Gaussian fits to eval loss as a function of repeat count.
%     Each panel fixes model size; each curve corresponds to an overtraining multiplier.
%     The fitted peak gives $\Rep^{\mathrm{peak}}$, the repeat count at which eval loss is largest for that $(N, \OT)$ sweep.
%     Across all model sizes, eval loss is maximized at an intermediate repeat count rather than at either extreme.
%   }
%   \label{fig:gaussian-fits-loss-r}
% \end{figure}

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=\linewidth]{scaling_law_allOT_four_views_loglog-1.png}
%   \caption{
%     Scaling laws for the peak-damage regime.
%     Top row: the repeat count at peak eval loss, $\Rep^{\mathrm{peak}}$, decreases with model size (left) and compute (right).
%     Bottom row: the repeated-pool size at peak eval loss, $\Dr^{\mathrm{peak}}$, increases with both.
%     Larger training runs are most damaged by larger repeated pools that need fewer passes to produce peak degradation.
%   }
%   \label{fig:peak-scaling-laws}
% \end{figure}








% A small value of $\Rep$ means that the repeated-token budget is spread over a larger pool of examples, and vice versa. This setup lets us identify the repeated-pool size and repeat count associated with the largest eval loss.  

% For each fixed $(N, \mathrm{OT})$ sweep, we fit a Gaussian-shaped peak to the loss curve as a function of repeat count.
% We fit the curve in the log-spaced repeat coordinate, but write the fitted peak generically as
% \[
% L(x)
% =
% b
% +
% A \exp\left(
%     -\frac{(x - \mu)^2}{2\sigma^2}
% \right),
% \]


% where $x$ is the transformed repeat coordinate, $b$ is the fitted baseline level, $A$ is the peak height, $\mu$ is the peak location, and $\sigma$ is the peak width.
% The fitted peak location gives $\Rep^{\mathrm{peak}}$, the repeat count at which eval loss is largest.

% Figure~\ref{fig:gaussian-fits-loss-r} shows the fitted curves overlaid on eval loss for each model size and overtraining multiplier.
% Across the fitted sweeps, eval loss increases with repetition, reaches a peak, and then decreases at larger repeat counts.
% This peak-loss shape shows that the most damaging regime is intermediate.
% When $\Rep$ is small, the repeated-token budget is spread broadly and each repeated example receives limited extra weight.
% When $\Rep$ is very large, the repeated pool is extremely small.
% Peak eval loss occurs between these limits, when the repeated pool is large enough to affect generalization but concentrated enough to be strongly overrepresented.

% After extracting $\Rep^{\mathrm{peak}}$ from each fitted curve, we fit a scaling law for the peak location.
% Across model sizes and overtraining multipliers, the fitted relationship between peak repeat count and model size is
% \[
% \Rep^{\mathrm{peak}}
% =
% 9.33 \times 10^8 N^{-0.79}.
% \]

% This compute form estimates the repeat count most associated with peak eval loss at a given pretraining compute budget.


%   The repeat-count scaling law does not fully describe the repeated-data structure, because $\Rep$ and $\Dr$ move in opposite directions.
%   Using $\Dr=fT/\Rep$, we also fit the repeated-pool size at peak eval loss:
%   \[
%       \Dr^{\mathrm{peak}}
%       =
%       1.87\times 10^{-8} N^{1.67},
%   \]
%   and equivalently,
%   \[
%       \Dr^{\mathrm{peak}}
%       =
%       4.00\times 10^{-11} C^{0.89}.
%   \]
%   These positive exponents show that the repeated pool associated with peak eval loss grows with model size and compute.
%   Larger models are most damaged by larger repeated pools, but those repeated pools need fewer repeats to produce the largest eval loss.

%   Figure~\ref{fig:peak-scaling-laws} summarizes these fitted peak-location laws.
%   The top panels show that $\Rep^{\mathrm{peak}}$ decreases with model size and compute.
%   The bottom panels show that $\Dr^{\mathrm{peak}}$ increases with model size and compute.
%   Together, these trends answer which repeat regime is worst: peak eval loss occurs when the repeated pool is neither broad and lightly repeated nor tiny and heavily repeated, but instead
%   lies at an intermediate scale that grows with model size and compute.

%   \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{gaussian_fits_loss_vs_R_image18-1.png}
%     \caption{
%     Gaussian fits to eval loss as a function of repeat count.
%     Each panel fixes model size, and each curve corresponds to an overtraining multiplier.
%     The fitted peak gives $\Rep^{\mathrm{peak}}$, the repeat count where eval loss is largest for that $(N,\OT)$ sweep.
%     Across model sizes, eval loss is maximized at an intermediate repeat count rather than at either endpoint of the sweep.
%     }
%     \label{fig:gaussian-fits-loss-r}
%   \end{figure}












%   The repeat-count scaling law does not fully describe the repeated-data structure, because $\Rep$ and $\Dr$ move in opposite directions.
%   Using $\Dr=fT/\Rep$, we also fit the repeated-pool size at peak eval loss:
%   \[
%       \Dr^{\mathrm{peak}}
%       =
%       1.87\times 10^{-8} N^{1.67},
%   \]
%   and equivalently,
%   \[
%       \Dr^{\mathrm{peak}}
%       =
%       4.00\times 10^{-11} C^{0.89}.
%   \]
%   These positive exponents show that the repeated pool associated with peak eval loss grows with model size and compute.
%   Larger models are most damaged by larger repeated pools, but those repeated pools need fewer repeats to produce the largest eval loss.

%   Figure~\ref{fig:peak-scaling-laws} summarizes these fitted peak-location laws.
%   The top panels show that $\Rep^{\mathrm{peak}}$ decreases with model size and compute.
%   The bottom panels show that $\Dr^{\mathrm{peak}}$ increases with model size and compute.
%   Together, these trends answer which repeat regime is worst: peak eval loss occurs when the repeated pool is neither broad and lightly repeated nor tiny and heavily repeated, but instead
%   lies at an intermediate scale that grows with model size and compute.
















